Unsupervised Learning via Meta-Learning

A central goal of unsupervised learning is to acquire representations from unlabeled data or experience that can be used for more effective learning of downstream tasks from modest amounts of labeled data. Many prior unsupervised learning works aim to do so by developing proxy objectives based on reconstruction, disentanglement, prediction, and other metrics. Instead, we develop an unsupervised meta-learning method that explicitly optimizes for the ability to learn a variety of tasks from small amounts of data. To do so, we construct tasks from unlabeled data in an automatic way and run meta-learning over the constructed tasks. Surprisingly, we find that, when integrated with meta-learning, relatively simple task construction mechanisms, such as clustering embeddings, lead to good performance on a variety of downstream, human-specified tasks. Our experiments across four image datasets indicate that our unsupervised meta-learning approach acquires a learning algorithm without any labeled data that is applicable to a wide range of downstream classification tasks, improving upon the embedding learned by four prior unsupervised learning methods.

==> figures/results_celeba_ours.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=2.2cm,
        height=4cm,
        scale only axis,
        ybar,
        ylabel={\% classification accuracy},
        ylabel style={yshift=-5pt, font=\footnotesize},
        symbolic x coords={2-way 5-shot},
        xtick=data,
        xticklabel style={yshift=2pt},
        %nodes near coords={\hspace{1pt} \pgfmathprintnumber[fixed zerofill, precision=1]{\pgfplotspointmeta}},
        ybar=0pt,
        bar width=6pt,
        every node near coord/.append style={rotate=90, anchor=west, font=\tiny},
        legend cell align={left},
        legend style={draw=none, fill=none, at={(1, 0)}, anchor=south west, column sep=5pt},
        legend columns=1,
        axis x line*=bottom,
        axis y line*=left,
        xtick style={/pgfplots/major tick length=0pt},
        ytick style={/pgfplots/major tick length=0pt},
        title={CelebA},
        title style={xshift=75pt, yshift=-10pt},
        ymax=100,
        ymin=50
    ]
    
    % DeepCluster-CACTUs-UMAML p=50
    \addplot+[
        color=blue,
        fill=blue!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 73.79) +- (1.01, 1.01)
    };
    
    % DeepCluster-LR
    \addplot+[
        color=blue,
        fill=blue!25,
        postaction={pattern=north east lines, pattern color=blue},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 59.57) +- (0.98, 0.98)
    };
    
    % DeepCluster-NN
    \addplot+[
        color=blue,
        fill=blue!25,
        postaction={pattern=horizontal lines, pattern color=blue},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 61.47) +- (0.99, 0.99)
    };
    
    % BiGAN-CACTUs-UMAML p=50
    \addplot+[
        color=violet,
        fill=violet!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 74.41) +- (0.83, 0.83)
    };
    
    % BiGAN-LR
    \addplot+[
        color=violet,
        fill=violet!25,
        postaction={pattern=north east lines, pattern color=violet},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 58.44) +- (0.90, 0.90)
    };
    
    % BiGAN-NN
    \addplot+[
        color=violet,
        fill=violet!25,
        postaction={pattern=horizontal lines, pattern color=violet},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 56.15) +- (0.89, 0.89)
    };
    
    % Scratch
    \addplot+[
        color=gray,
        fill=gray!50,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 63.19) +- (1.06, 1.06)
    };
    
    % Oracle-Control-MAML
    \addplot+[
        color=black,
        fill=white,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        (2-way 5-shot, 87.10) +- (0.85, 0.85)
    };
    
    
    \legend{
        \small DeepCluster-\method -MAML (ours), 
        \small DeepCluster + linear classifier,
        \small DeepCluster + nearest neighbors,
        \small BiGAN-\method -MAML (ours),
        \small BiGAN + linear classifier,
        \small BiGAN + nearest neighbors,
        \small Training from scratch,
        \small Oracle-MAML (control)
    }

    \end{axis}
\end{tikzpicture}

==> figures/results_miniimagenet_ours.tex <==
\begin{tikzpicture}
 \vspace{-0.3cm}
    \begin{axis}[
        width=7.5cm,
        height=4cm,
        scale only axis,
        ylabel={\% classification accuracy},
        ylabel style={yshift=-5pt, font=\footnotesize},
        xlabel={(way, shot)},
        xlabel style={font=\footnotesize, yshift=5pt},
        symbolic x coords={{(5, 1)}, {(5, 5)}, {(5, 20)}, {(5, 50)}},
        xtick=data,
        xticklabel style={yshift=2pt},
        %nodes near coords={\hspace{1pt} \pgfmathprintnumber[fixed zerofill, precision=1]{\pgfplotspointmeta}},
        bar width=6pt,
        ybar=0pt,
        every node near coord/.append style={rotate=90, anchor=west, font=\tiny},
        legend cell align={left},
        legend style={draw=none, fill=none, at={(1, 0)}, anchor=south west, column sep=5pt},
        legend columns=1,
        enlarge x limits=0.17,
        axis x line*=bottom,
        axis y line*=left,
        xtick style={/pgfplots/major tick length=0pt},
        ytick style={/pgfplots/major tick length=0pt},
        title={miniImageNet},
        title style={xshift=70pt,yshift=-10pt},
        ymax=100,
    ]
    
    % DeepCluster-CACTUs-UMAML p=50
    \addplot+[
        color=blue,
        fill=blue!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 39.90) +- (0.74, 0.74)
        ({(5, 5)}, 53.97) +- (0.70, 0.70)
        ({(5, 20)}, 63.84) +- (0.70, 0.70)
        ({(5, 50)}, 69.64) +- (0.63, 0.63)
    };
    
    % DeepCluster-LR
    \addplot+[
        color=blue,
        fill=blue!25,
        postaction={pattern=north east lines, pattern color=blue},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 29.44) +- (1.22, 1.22)
        ({(5, 5)}, 39.79) +- (0.64, 0.64)
        ({(5, 20)}, 56.19) +- (0.43, 0.43)
        ({(5, 50)}, 65.28) +- (0.34, 0.34)
    };
    
    % DeepCluster-NN
    \addplot+[
        color=blue,
        fill=blue!25,
        postaction={pattern=horizontal lines, pattern color=blue},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 28.90) +- (1.25, 1.25)
        ({(5, 5)}, 42.25) +- (0.67, 0.67)
        ({(5, 20)}, 56.44) +- (0.43, 0.43)
        ({(5, 50)}, 63.90) +- (0.38, 0.38)
    };
    
    % BiGAN-CACTUs-UMAML p=50
    \addplot+[
        color=violet,
        fill=violet!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 36.24) +- (0.74, 0.74)
        ({(5, 5)}, 51.28) +- (0.68, 0.68)
        ({(5, 20)}, 61.33) +- (0.67, 0.67)
        ({(5, 50)}, 66.91) +- (0.68, 0.68)
    };
    
    % BiGAN-LR
    \addplot+[
        color=violet,
        fill=violet!25,
        postaction={pattern=north east lines, pattern color=violet},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 27.08) +- (1.24, 1.24)
        ({(5, 5)}, 33.91) +- (0.64, 0.64)
        ({(5, 20)}, 44.00) +- (0.45, 0.45)
        ({(5, 50)}, 50.41) +- (0.37, 0.37)
    };
    
    % BiGAN-NN
    \addplot+[
        color=violet,
        fill=violet!25,
        postaction={pattern=horizontal lines, pattern color=violet},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 25.56) +- (1.08, 1.08)
        ({(5, 5)}, 31.10) +- (0.63, 0.63)
        ({(5, 20)}, 37.31) +- (0.40, 0.40)
        ({(5, 50)}, 43.60) +- (0.37, 0.37)
    };
    
    % Scratch
    \addplot+[
        color=gray,
        fill=gray!50,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 27.59) +- (0.59, 0.59)
        ({(5, 5)}, 38.48) +- (0.66, 0.66)
        ({(5, 20)}, 51.53) +- (0.72, 0.72)
        ({(5, 50)}, 59.63) +- (0.74, 0.74)
    };
    
    % Oracle-Control-MAML
    \addplot+[
        color=black,
        fill=white,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 46.81) +- (0.77, 0.77)
        ({(5, 5)}, 62.13) +- (0.72, 0.72)
        ({(5, 20)}, 71.03) +- (0.69, 0.69)
        ({(5, 50)}, 75.54) +- (0.62, 0.62)
    };

    \legend{
        \small DeepCluster-\method -MAML (ours), 
        \small DeepCluster + linear classifier,
        \small DeepCluster + nearest neighbors,
        \small BiGAN-\method -MAML (ours),
        \small BiGAN + linear classifier,
        \small BiGAN + nearest neighbors,
        \small Training from scratch,
        \small Oracle-MAML (control)
    }

    % \legend{Far,Near}
    \end{axis}
    \vspace{-0.3cm}
\end{tikzpicture}

==> figures/results_miniimagenet_task_generation.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=4.5cm,
        height=4cm,
        scale only axis,
        ybar,
        ylabel={\% classification accuracy},
        ylabel style={yshift=-5pt, font=\footnotesize},
        bar width=6pt,
        xlabel={(way, shot)},
        xlabel style={font=\footnotesize, yshift=5pt},
        xticklabel style={yshift=2pt},
        symbolic x coords={{(5, 1)}, {(5, 5)}, {(5, 20)}, {(5, 50)}},
        xtick=data,
        %nodes near coords={\pgfmathprintnumber[fixed zerofill, precision=1]{\pgfplotspointmeta}},
        ybar=0pt,
        every node near coord/.append style={rotate=90, anchor=west, font=\tiny},
        legend columns=1,
        legend cell align={left},
        legend style={draw=none, fill=none, at={(-0.1,-0.2)}, anchor=north west, column sep=5pt},
        enlarge x limits=0.2,
        axis x line*=bottom,
        axis y line*=none,
        xtick style={/pgfplots/major tick length=0pt},
        ytick style={/pgfplots/major tick length=0pt},
        ymax=100,
        title={miniImageNet},
    ]
    % DeepCluster-CACTUs-UMAML p=50
    \addplot+[
        color=blue,
        fill=blue!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 39.90) +- (0.74, 0.74)
        ({(5, 5)}, 53.97) +- (0.70, 0.70)
        ({(5, 20)}, 63.84) +- (0.70, 0.70)
        ({(5, 50)}, 69.64) +- (0.63, 0.63)
    };
    
    % DeepCluster-CACTUs-UMAML p=1
    \addplot+[
        color=blue,
        fill=blue!25,
        postaction={pattern=dots, pattern color=blue},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 38.75) +- (0.70, 0.70)
        ({(5, 5)}, 52.73) +- (0.72, 0.72)
        ({(5, 20)}, 62.72) +- (0.69, 0.69)
        ({(5, 50)}, 67.77) +- (0.62, 0.62)
    };
    
    % DeepCluster-H-UMAML m=0.1
    \addplot+[
        color=blue,
        fill=white,
        postaction={pattern=grid, pattern color=blue},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 35.85) +- (0.66, 0.66)
        ({(5, 5)}, 49.54) +- (0.72, 0.72)
        ({(5, 20)}, 60.68) +- (0.69, 0.69)
        ({(5, 50)}, 65.55) +- (0.66, 0.66)
    };
    
    % DeepCluster-H-UMAML m=0
    \addplot+[
        color=blue,
        fill=white,
        postaction={pattern=crosshatch, pattern color=blue},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 20.02) +- (0.06, 0.06)
        ({(5, 5)}, 20.01) +- (0.01, 0.01)
        ({(5, 20)}, 20.00) +- (0.01, 0.01)
        ({(5, 50)}, 20.01) +- (0.02, 0.02)
    };

    \legend{DeepCluster-\method -MAML $P=50$, 
            DeepCluster-\method -MAML $P=1$, 
            DeepCluster-Hyperplanes-UMAML $m=0.1$, 
            DeepCluster-Hyperplanes-UMAML $m=0$}
    \end{axis}
\end{tikzpicture}

==> figures/results_omniglot_ours.tex <==
\todo{need to update numbers for 20-to-5} %%KH.09.24 
\begin{tikzpicture}
\vspace{-0.2cm}
    \begin{axis}[
        width=7.5cm,
        height=4cm,
        scale only axis,
        ybar,
        ylabel={\% classification accuracy},
        ylabel style={yshift=-5pt, font=\footnotesize},
        xlabel={(way, shot)},
        xlabel style={font=\footnotesize, yshift=5pt},
        symbolic x coords={{(5, 1)}, {(5, 5)}, {(20, 1)}, {(20, 5)}},
        xtick=data,
        xticklabel style={yshift=2pt},
        %nodes near coords={\hspace{1pt} \pgfmathprintnumber[fixed zerofill, precision=1]{\pgfplotspointmeta}},
        ybar=0pt,
        bar width=6pt,
        every node near coord/.append style={rotate=90, anchor=west, font=\tiny},
        legend cell align={left},
        legend style={draw=none, fill=none, at={(1, 0)}, anchor=south west, column sep=5pt},
        legend columns=1,
        enlarge x limits=0.17,
        axis x line*=bottom,
        axis y line*=left,
        xtick style={/pgfplots/major tick length=0pt},
        ytick style={/pgfplots/major tick length=0pt},
        title={Omniglot},
        title style={xshift=70pt},
        ymax=100,
    ]
    
    % ACAI-CACTUs-UMAML p=100
    \addplot+[
        color=teal,
        fill=teal,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 68.73) +- (0.80, 0.80)
        ({(5, 5)}, 87.90) +- (0.51, 0.51)
        ({(20, 1)}, 48.09) +- (0.41, 0.41)
        ({(20, 5)}, 73.36) +- (0.34, 0.34)
    };
    
    % % ACAI-CACTUs-UMAML p=1
    % \addplot+[
    %     error bars/.cd,
    %         y dir=both, y explicit,
    % ] coordinates {
    %     ({(5, 1)}, 66.52) +- (0.85, 0.85)
    %     ({(5, 5)}, 86.18) +- (0.54, 0.54)
    %     ({(20, 1)}, 45.04) +- (0.41, 0.41)
    %     ({(20, 5)}, 69.14) +- (0.36, 0.36)
    % };
    
    % ACAI-LR
    \addplot+[
        color=teal,
        fill=teal!25,
        postaction={pattern=north east lines, pattern color=teal},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 61.08) +- (1.32, 1.32)
        ({(5, 5)}, 81.82) +- (0.58, 0.58)
        ({(20, 1)}, 43.20) +- (0.69, 0.69)
        ({(20, 5)}, 66.33) +- (0.36, 0.36)
    };
    
    % ACAI-NN
    \addplot+[
        color=teal,
        fill=teal!25,
        postaction={pattern=horizontal lines, pattern color=teal},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 57.46) +- (1.35, 1.35)
        ({(5, 5)}, 81.16) +- (0.57, 0.57)
        ({(20, 1)}, 39.73) +- (0.38, 0.38)
        ({(20, 5)}, 66.38) +- (0.36, 0.36)
    };
    
    % BiGAN-CACTUs-UMAML p=100
    \addplot+[
        color=violet,
        fill=violet!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 57.17) +- (0.77, 0.77)
        ({(5, 5)}, 77.38) +- (0.57, 0.57)
        ({(20, 1)}, 35.56) +- (0.36, 0.36)
        ({(20, 5)}, 58.62) +- (0.38, 0.38)
    };
    
    % % BiGAN-CACTUs-UMAML p=1
    % \addplot+[
    %     error bars/.cd,
    %         y dir=both, y explicit,
    % ] coordinates {
    %     ({(5, 1)}, 55.67) +- (0.75, 0.75)
    %     ({(5, 5)}, 75.90) +- (0.58, 0.58)
    %     ({(20, 1)}, 32.44) +- (0.35, 0.35)
    %     ({(20, 5)}, 54.22) +- (0.39, 0.39)
    % };
    
    % BiGAN-LR
    \addplot+[
        color=violet,
        fill=violet!25,
        postaction={pattern=north east lines, pattern color=violet},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 48.28) +- (1.25, 1.25)
        ({(5, 5)}, 68.72) +- (0.66, 0.66)
        ({(20, 1)}, 27.80) +- (0.61, 0.61)
        ({(20, 5)}, 46.70) +- (0.36, 0.36)
    };
    
    % BiGAN-NN
    \addplot+[
        color=violet,
        fill=violet!25,
        postaction={pattern=horizontal lines, pattern color=violet},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 49.55) +- (1.27, 1.27)
        ({(5, 5)}, 68.06) +- (0.71, 0.71)
        ({(20, 1)}, 27.37) +- (0.33, 0.33)
        ({(20, 5)}, 46.70) +- (0.36, 0.36)
    };
    
    % Scratch
    \addplot+[
        color=gray,
        fill=gray!50,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 52.50) +- (0.84, 0.84)
        ({(5, 5)}, 74.78) +- (0.69, 0.69)
        ({(20, 1)}, 24.91) +- (0.33, 0.33)
        ({(20, 5)}, 47.62) +- (0.44, 0.44)
    };
    
    % Oracle-Control-MAML
    \addplot+[
        color=black,
        fill=white,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 94.46) +- (0.35, 0.35)
        ({(5, 5)}, 98.83) +- (0.12, 0.12)
        ({(20, 1)}, 84.60) +- (0.32, 0.32)
        ({(20, 5)}, 96.29) +- (0.13, 0.13)
    };
    
    \legend{
        \small ACAI-\method -MAML (ours), 
        \small ACAI + linear classifier,
        \small ACAI + nearest neighbors,
        \small BiGAN-\method -MAML (ours),
        \small BiGAN + linear classifier,
        \small BiGAN + nearest neighbors,
        \small Training from scratch,
        \small Oracle-MAML (control)
    }
    \end{axis}
\end{tikzpicture}

==> figures/results_omniglot_task_generation.tex <==
\todo{need to update numbers for 20-to-5} %%KH.09.24 
\begin{tikzpicture}
    \begin{axis}[
        width=5.5cm,
        height=4cm,
        scale only axis,
        ymin=0,
        ybar,
        ylabel={\% classification accuracy},
        ylabel style={yshift=-5pt, font=\footnotesize},
        xlabel={(way, shot)},
        xlabel style={font=\footnotesize, yshift=5pt},
        xticklabel style={yshift=2pt},
        symbolic x coords={{(5, 1)}, {(5, 5)}, {(20, 1)}, {(20, 5)}},
        xtick=data,
        %nodes near coords={\hspace{1pt} \pgfmathprintnumber[fixed zerofill, precision=1]{\pgfplotspointmeta}},
        ybar=0pt,
        bar width=6pt,
        every node near coord/.append style={rotate=90, anchor=west, font=\tiny},
        legend cell align={left},
        legend style={draw=none, fill=none, at={(-0.1,-0.2)}, anchor=north west, column sep=5pt},
        legend columns=1,
        enlarge x limits=0.2,
        axis x line*=bottom,
        axis y line*=left,
        xtick style={/pgfplots/major tick length=0pt},
        ytick style={/pgfplots/major tick length=0pt},
        ymax=100,
        title={Omniglot},
    ]
    % order:    better-embedding cactus p=50,
    %           better-embedding cactus p=1,
    %           better-embedding H, m as much as possible
    %           better-embedding H, m=0
    %           random
    % ACAI-CACTUs-UMAML p=100
    \addplot+[
        color=teal,
        fill=teal!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 68.73) +- (0.80, 0.80)
        ({(5, 5)}, 87.90) +- (0.51, 0.51)
        ({(20, 1)}, 48.09) +- (0.41, 0.41)
        ({(20, 5)}, 73.36) +- (0.34, 0.34)
    };
    % ACAI-CACTUs-UMAML p=1
    \addplot+[
        color=teal,
        fill=teal!25,
        postaction={pattern=dots, pattern color=teal},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 66.52) +- (0.85, 0.85)
        ({(5, 5)}, 86.18) +- (0.54, 0.54)
        ({(20, 1)}, 45.04) +- (0.41, 0.41)
        ({(20, 5)}, 69.14) +- (0.36, 0.36)
    };
    % ACAI-H-UMAML m=1.2
    \addplot+[
        color=teal,
        fill=white,
        postaction={pattern=grid, pattern color=teal},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 61.30) +- (0.83, 0.83)
        ({(5, 5)}, 80.22) +- (0.63, 0.63)
        ({(20, 1)}, 41.86) +- (0.38, 0.38)
        ({(20, 5)}, 65.23) +- (0.37, 0.37)
    };
    % ACAI-H-UMAML m=0
    \addplot+[
        color=teal,
        fill=white,
        postaction={pattern=crosshatch, pattern color=teal},
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 61.55) +- (0.84, 0.84)
        ({(5, 5)}, 80.14) +- (0.64, 0.64)
        ({(20, 1)}, 39.30) +- (0.37, 0.37)
        ({(20, 5)}, 63.18) +- (0.38, 0.38)
    };
    % Random-UMAML
    \addplot+[
        color=black,
        fill=black!75,
        error bars/.cd,
            y dir=both, y explicit,
    ] coordinates {
        ({(5, 1)}, 25.99) +- (0.73, 0.73)
        ({(5, 5)}, 25.74) +- (0.69, 0.69)
        ({(20, 1)}, 6.51) +- (0.18, 0.18)
        ({(20, 5)}, 6.74) +- (0.18, 0.18)
    };
    \legend{ACAI-\method -MAML $P=100$, 
            ACAI-\method -MAML $P=1$, 
            ACAI-Hyperplanes-UMAML $m=1.2$, 
            ACAI-Hyperplanes-UMAML $m=0$, 
            Random-UMAML}
    \end{axis}
\end{tikzpicture}

==> tables/celeba_ours.tex <==
\begin{table}[htb]
\footnotesize
\caption{Results of unsupervised learning on CelebA images, averaged over 1000 downstream attribute recognition tasks. \method{} experiments use $k=500$ clusters for each of $P=50$ partitions. Embedding cluster matching uses the same $k$. For complete results with confidence intervals, see Table~\ref{table:celeba} in Appendix~\ref{app:tables}.}
\vspace{-0.3cm}
\label{table:celeba_ours}
\begin{center}
\begin{tabular}{@{}lcc@{}}
\toprule
Algorithm \textbackslash{} (way, shot) & (2, 5) \\ 
\midrule
Training from scratch & 63.19\% \\
\cdashlinelr{1-2}
BiGAN $k_\text{nn}$-nearest neighbors & 56.15\% \\
BiGAN linear classifier & 58.44\% \\
BiGAN MLP with dropout & 56.26\% \\
BiGAN cluster matching & 56.20\% \\
BiGAN \method{}-MAML (ours) & \textbf{74.98\%} \\
BiGAN \method{}-ProtoNets (ours) & 65.58\% \\
\cdashlinelr{1-2}
DeepCluster $k_\text{nn}$-nearest neighbors & 61.47\% \\
DeepCluster linear classifier & 59.57\% \\
DeepCluster MLP with dropout & 60.65\% \\
DeepCluster cluster matching & 51.51\% \\
DeepCluster \method{}-MAML (ours) & \textbf{73.79\%} \\
DeepCluster \method{}-ProtoNets (ours) & \textbf{74.15\%} \\
\midrule
\oracle{} (control) & 87.10\% \\
Oracle-ProtoNets (control) & 85.13\% \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-0.3cm}
\end{table}

==> tables/miniimagenet_ours.tex <==
\begin{table}[htb]
\footnotesize
\caption{Results of unsupervised learning on miniImageNet images, averaged over 1000 downstream classification tasks. \method{} experiments use $k=500$ for each of $P=50$ partitions. Embedding cluster matching uses the same $k$. Table~\ref{table:miniimagenet} in Appendix~\ref{app:tables}.} 
\label{table:miniimagenet_ours}
\vspace{-0.3cm}
\begin{center}
\begin{tabular}{@{}lcccc@{}}
\toprule
Algorithm \textbackslash{} (way, shot) & (5, 1) & (5, 5) & (5, 20) & (5, 50) \\ 
\midrule
Training from scratch & 27.59\% & 38.48\% & 51.53\% & 59.63\% \\
\cdashlinelr{1-5}
BiGAN $k_\text{nn}$-nearest neighbors & 25.56\% & 31.10\% & 37.31\% & 43.60\% \\
BiGAN linear classifier & 27.08\% & 33.91\% & 44.00\% & 50.41\% \\
BiGAN MLP with dropout & 22.91\% & 29.06\% & 40.06\% & 48.36\% \\
BiGAN cluster matching & 24.63\% & 29.49\% & 33.89\% & 36.13\% \\
BiGAN \method -MAML (ours) & 36.24\% & 51.28\% & 61.33\% & 66.91\% \\
BiGAN \method{}-ProtoNets (ours) & 36.62\% & 50.16\% & 59.56\% & 63.27\% \\
\cdashlinelr{1-5}
DeepCluster $k_\text{nn}$-nearest neighbors & 28.90\% & 42.25\% & 56.44\% & 63.90\% \\
DeepCluster linear classifier & 29.44\% & 39.79\% & 56.19\% & 65.28\% \\
DeepCluster MLP with dropout & 29.03\% & 39.67\% & 52.71\% & 60.95\% \\
DeepCluster cluster matching & 22.20\% & 23.50\% & 24.97\% & 26.87\% \\
DeepCluster \method -MAML (ours) & \textbf{39.90\%} & \textbf{53.97\%} & \textbf{63.84\%} & \textbf{69.64\%} \\
DeepCluster \method{}-ProtoNets (ours) & \textbf{39.18\%} & \textbf{53.36\%} & 61.54\% & 63.55\% \\
\midrule
Oracle-MAML (control) & 46.81\% & 62.13\% & 71.03\% & 75.54\% \\
Oracle-ProtoNets (control) & 46.56\% & 62.29\% & 70.05\% & 72.04\% \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-0.3cm}
\end{table}
